MESH: A Flexible Distributed Hypergraph Processing System

With the rapid growth of large online social networks, the ability to analyze large-scale social structure and behavior has become critically important, and this has led to the development of several scalable graph processing systems. In reality, however, social interaction takes place not only between pairs of individuals as in the graph model, but rather in the context of multi-user groups. Research has shown that such group dynamics can be better modeled through a more general hypergraph model, resulting in the need to build scalable hypergraph processing systems. In this paper, we present MESH, a flexible distributed framework for scalable hypergraph processing. MESH provides an easy-to-use and expressive application programming interface that naturally extends the think like a vertex model common to many popular graph processing systems. Our framework provides a flexible implementation based on an underlying graph processing system, and enables different design choices for the key implementation issues of partitioning a hypergraph representation. We implement MESH on top of the popular GraphX graph processing framework in Apache Spark. Using a variety of real datasets and experiments conducted on a local 8-node cluster as well as a 65-node Amazon AWS testbed, we demonstrate that MESH provides flexibility based on data and application characteristics, as well as scalability with cluster size. We further show that it is competitive in performance to HyperX, another hypergraph processing system based on Spark, while providing a much simpler implementation (requiring about 5X fewer lines of code), thus showing that simplicity and flexibility need not come at the cost of performance.

==> discussion.tex <==
\section{Discussion \& Future Work}
\label{sec:discussion}

We plan to explore a number of enhancements to \mesh{}, in terms of both its API
and its implementation.

\paragraph{Automatic Partitioning and Representation Selection}
We have demonstrated that there is no one-size-fits-all answer to the key
questions of how to represent a hypergraph, and how to partition that
representation for distributed processing.
Instead, the best choice depends upon the particular hypergraph.

In some cases, analysts may focus on a single hypergraph or slowly
evolving versions of a single hypergraph (e.g., Facebook group structure,
Twitter followers, etc.).
In these cases, it is practical to invest some up-front effort in determining
the best representation and partitioning techniques.

In other cases, however, it may be necessary to process a varying set of
hypergraphs and applications on a single deployment.
In these cases, determining which representation and partitioning to use on a
case-by-case basis could quickly become tedious.
We are exploring approaches for automating this selection based on application
and data characteristics.
For example, our experiments in Section~\ref{sec:evaluation} showed that the
relative number of hyperedges and vertices in a hypergraph can influence which
of these sets should be partitioned and which should be cut.
It may be possible to train a model to predict an appropriate representation
and partitioning to (nearly) eliminate the need for manual selection of these
parameters.

\paragraph{Directed Hyperedges}
We currently model only undirected hyperedges; i.e., each hyperedge is simply a
set of vertices.
It may be useful to support directed hyperedges, where each hyperedge contains
one or more source vertices and one or more destination vertices.
The \mesh{} API would need to be extended to allow applications to differentiate
between sources and destinations, and the implementation would also need to be
extended to model this distinction.
Allowing this additional modeling flexibility would only increase the diversity
of data and applications that \mesh{} would be required to handle, and this may
further motivate future work on partitioning and representation techniques.

Note that HyperX exclusively models directed hypergraphs, with the
restrictions that 1) each hyperedge must contain at least one source
and at least one destination, and 2) the source and destination sets must
be disjoint.
Undirected hyperedges can be emulated by arbitrarily partitioning each
hyperedge into source and destination subsets and ignoring the distinction
between source and vertex in the application code.
Unfortunately, these restrictions effectively prohibit hyperedges with
cardinality 1, which for example is required to model single-author papers in
our dblp dataset.
A more general model would allow the source and destination sets to overlap.

\paragraph{Asynchronous Computation}
In its current form, the \mesh{} API is purely synchronous; all vertex computation
finishes before the next round of hyperedge computation begins, and so on.
This is similar to the Pregel and GraphX models, and facilitates simpler
programs and system implementations, though possibly at the cost of slower
convergence~\cite{low2010}.
Supporting asynchronous computation would impact both the API and
implementation, and may restrict the choice of implementation platform.



%\paragraph{Alternative Representations}
%E.g., multigraph.

%\paragraph{Pluggable Implementations}
%E.g., run on RDBMS~\cite{fan2015}, \mesh{}-on-HyperX.


==> prototype.tex <==
\section{\mesh{} Prototype}

We have implemented a \mesh{} prototype on top of the GraphX~\cite{gonzalez2014} graph processing system, which
itself is implemented
on top of Apache Spark~\cite{zaharia2012}, the wildly
popular and rapidly growing general-purpose data-intensive computing platform.
Spark achieves good performance---especially on the iterative workloads that
graph and hypergraph computing require---through its novel Resilient Distributed Dataset
abstraction, which enables fault-tolerant distributed in-memory computing.

\subsection{Representation}

\todo{AC: Add more details.}
GraphX provides a graph representation consisting of vertices and edges represented as RDDs.
We provide...
We can represent a hypergraph using a clique representation by mapping each hyperedge to a clique of its incident vertices. Similarly, we can represent a hypergraph as a bipartite graph by creating edges between vertices and their hyperedges.
Interestingly, GraphX also supports a multi-graph representation, however, we have not found it to be useful for our purposes.

\subsection{Partitioning}

GraphX uses an edge-partitioning algorithm for partitioning the graph across machines.
In GraphX, the \mintinline{scala}{PartitionStrategy} is responsible for
assigning each graph edge to a partition.
GraphX uses this assignment to partition the set of edges, while replicating
each vertex to every partition that contains edges incident on that
vertex.
In GraphX, the \mintinline{scala}{PartitionStrategy} considers each edge in
isolation, as in Listing~\ref{listing:graphx-old}.
\begin{listing}[htbp]
  \begin{minted}[fontsize=\scriptsize]{scala}
def getPartition(
  src: VertexId,
  dst: VertexId,
  numPart: PartitionId): PartitionId
  \end{minted}
  %\vspace{0.5em}
  \caption{Original GraphX partitioning abstraction.\label{listing:graphx-old}}
\end{listing}

We use the inbuilt GraphX partitioning algorithms to implement the baseline Random partitioning algorithms described above. 
Our Greedy and Hybrid algorithms, however, require a broader view of the graph
(to compute ``overlap'' and degree/cardinality, respectively).
To satisfy this requirement, we extend the
\mintinline{scala}{PartitionStrategy} by adding a new
\mintinline{scala}{getPartitionedEdgeRDD} method that allows partitioning
decisions to be made with awareness of the full graph, as shown in
Listing~\ref{listing:graphx-new}.

\begin{listing}[htbp]
  \begin{minted}[fontsize=\scriptsize]{scala}
def getPartitionedEdgeRDD[VD, ED](
  graph: Graph[VD, ED],
  numPartitions: PartitionId,
  degreeCutoff: Int): RDD[(PartitionId, (VertexId, VertexId, ED))]
  \end{minted}
  %\vspace{0.5em}
  \caption{Additional GraphX partitioning abstraction.\label{listing:graphx-new}}
\end{listing}

% TODO - this is a very poorly designed API.  Its intentions would be much clearer if
% it returned RDD[(((VertexId, VertexId), PartitionId)], which we could
% basically view as a map from (srcId, dstId) --> partition,
% just as getPartition can be viewed in the original API.
% Besides, a partitioning algorithm should absolutely NOT be allowed to
% change the attributes of the edges, as this API implicitly allows.
% See also comments in source code.  Propose a better API in the paper, and
% fix it in our code before open-sourcing.

